FLAME: A Self-Adaptive Auto-labeling System for Heterogeneous Mobile Processors

How to accurately and efficiently label data on a mobile device is critical for the success of training machine learning models on mobile devices. Auto-labeling data on mobile devices is challenging, because data is usually incrementally generated and there is possibility of having unknown labels. Furthermore, the rich hardware heterogeneity on mobile devices creates challenges on efficiently executing auto-labeling workloads. In this paper, we introduce Flame, an auto-labeling system that can label non-stationary data with unknown labels. Flame includes a runtime system that efficiently schedules and executes auto-labeling workloads on heterogeneous mobile processors. Evaluating Flame with eight datasets on a smartphone, we demonstrate that Flame enables auto-labeling with high labeling accuracy and high performance.

==> content/overview.tex <==
\section{Overview {\color{red}(0.5 pages)}}
\label{sec:overview}
The design of \name includes both algorithm and software system. Figure~\ref{fig:overview} gives an overview of \name.

Our auto-labeling algorithm enables automatic labeling for unlabeled data to achieve three goals: (1) assign labels to unlabeled data using labels in $Y$ ($Y$ is a set of existing labels); (2) a new label can be immediately detected; and (3) heuristic functions for data labeling can be self-adapted over a non-stationary unlabeled data.


As Figure~\ref{fig:overview} shows, the input of \name is a limited number of labeled data. 
\textcolor{dong}{(Please re-write the following paragraph. Summarize the major ideas and make sure your summary can be easily understood.)}
Each heuristic function may cover only a small portion of the data to be labeled, there is a trade off between coverage and the labeling quality. Thus, here we build a number of initial heuristic functions though the Heuristic Function Generator. The built heuristic functions are used for labeling for a large number of unlabeled data. As the unlabeled data dynamically generated, a novel label $y^{*} \in Y{'} \wedge y^{*} \notin Y$ may appear over this non-stationary process. Thus, our system maintains a Heuristics Self-adptation mechanism to detect whether a novel label $y^{*}$ appears and immediately update the parameters related with each heuristic function. Each heuristic function generates a weak labeling result and a real value number which indicates the labeling confidence for each coming data, then, the Labeling Aggregator uses the ensemble technique to get a robust labeling result through aggregating the confidence value generated by each heuristic function. Furthermore, the aggregated confidence value is checked through a verifier using a pre-defined parameter $\tau$. If the aggregated confidence value is larger than $\tau$, the label will be assigned to the corresponding unlabeled data, otherwise, this unlabeled data needs to wait for further checking. 


%The main idea of this paper is to automatic labeling for the unlabeled data such that: $1)$ the labels of  unlabeled data in $Y$ can be correctly assigned; $2)$ a novel label $y^{*} \in Y^{'}-Y$, where  $y^{*} \in Y{'} \wedge y^{*} \notin Y$, can be immediately detected, and $3)$ heuristic functions for data labeling can be self-adapted over a non-stationary unlabeled data. As the figure 1 shows, the input of the system at the beginning is the limited number of the labeled data. Each heuristic function may cover only a small portion of the data to be labeled, there is a trade off between coverage and the labeling quality. Thus, here we build a number of initial heuristic functions though the Heuristic Function Generator. The built heuristic functions are used for labeling for a large number of unlabeled data. As the unlabeled data dynamically generated, a novel label $y^{*} \in Y{'} \wedge y^{*} \notin Y$ may appear over this non-stationary process. Thus, our system maintains a Heuristics Self-adptation mechanism to detect whether a novel label $y^{*}$ appears and immediately update the parameters related with each heuristic function. Each heuristic function generates a weak labeling result and a real value number which indicates the labeling confidence for each coming data, then, the Labeling Aggregator uses the ensemble technique to get a robust labeling result through aggregating the confidence value generated by each heuristic function. Furthermore, the aggregated confidence value is checked through a verifier using a pre-defined parameter $\tau$. If the aggregated confidence value is larger than $\tau$, the label will be assigned to the corresponding unlabeled data, otherwise, this unlabeled data needs to wait for further checking. 

Our system design includes a runtime system.
To , in the runtime system design, we propose the heterogeneity-aware kernel scheduling and parallelism optimization for heterogeneous mobile processors. As shown in Figure~\ref{fig:overview}, we first profile and characterize kernels. The profiling and characteristics of kernels are automatically processed online using the first few chunks of the auto-labeling model in \circled{5}. Aiming to optimize the hardware efficiency and address the straggler effect across kernels, we perform heterogeneity-aware kernel scheduling using several greedy-heuristic strategies based on the kernel profiling and features of mobile processors. 

%To , in the runtime system design, we propose the heterogeneity-aware kernel scheduling and parallelism optimization for heterogeneous mobile processors. As shown in Figure~\ref{fig:overview}, we first profile and characterize kernels. The profiling and characteristics of kernels are automatically processed online using the first few chunks of the auto-labeling model in \circled{5}. Aiming to optimize the hardware efficiency and address the straggler effect across kernels, we perform heterogeneity-aware kernel scheduling using several greedy-heuristic strategies based on the kernel profiling and features of mobile processors. 


To address the issues of straggler effect and load imbalance within a kernel, we propose a heterogeneity-aware intra-kernel division to dynamically divide the parallel kernel for heterogeneous mobile processors. We build two analytical prediction models based on the kernel profiling results, computational ability of heterogeneous mobile processors and features of auto-labeling model. One model predicts the optimal parallelism granularity of executing a kernel on homogeneous CPU cores. In order to achieve load balance of executing a kernel, another model provides the optimal percentage of dividing the workload of a kernel for heterogeneous mobile processors. In Figure~\ref{fig:overview}, we apply the kernel characteristics and profiling results for the approaches of heterogeneity-aware kernel scheduling and parallelism optimization in \circled{6} and employ the approaches in the heterogeneity-aware mobile runtime system in \circled{7}. In the auto-labeling phase, the runtime system obtain the output data from the labeling aggregator and verifier as input data in \circled{9}. The runtime system processes the input data and automatically generates the labels for all unlabeled data.

\begin{algorithm}[tb]
   \caption{Prototype Update and Incremental Heuristics}
   \label{alg:example}
\begin{algorithmic}
   \STATE {\bfseries Input:} data set $\mathcal{D}$ without labels, heuristic function set $\mathcal{H}$, current overall prototype set $\mathcal{P}$ for $\mathcal{H}$, labeling confidence threshold $\tau$, small buffer $\mathcal{B}$, current label set $\mathcal{L}$, threshold set $\Phi$ for $\mathcal{L}$ 
   \STATE {\bfseries Output:} updated prototypes $\mathbcal{P}$, updated label set $\mathcal{L}$  
   \REPEAT
   \STATE $matchedHeuristic = false$
   \FOR{$i=1$ {\bfseries to} $T=\lvert \mathcal{H} \rvert$}
   \STATE k = $\lvert \mathbbm{P_{i}} \rvert$   // $\mathbbm{P_{i}} \in \mathcal{P}$
   \STATE $d_{x,\mathbbm{P_{ij}}} = \min_{j=1}^{k}{\lVert f(x) - c_{ij} \rVert}_2^2$ // data point $x \in \mathcal{D}$ 
   \IF{$d_{x,\mathbbm{P_{ij}}} < \Phi_{i}$}
   \STATE $updatePrototype(\mathbbm{P_{ij}})$
   \STATE $calConfidence(\mathbbm{H_{i}}, x)$
   \STATE $matchedHeuristic = true$
   \ENDIF
   \ENDFOR
   \STATE Get the label of $x$ using Equation 2
   \IF{$matchedHeuristic = false$}
   \STATE $\mathcal{B} = \mathcal{B} \bigcup x$
   \ENDIF
   \STATE // Periodic check the buffer $\mathcal{B}$
   \FOR{$inst \in \mathcal{B}$}
   \IF{$q\_NSC(inst) > 1$}
   \STATE Get a set $\mathbcal{S}$ potentially with the same new label $\ell$
   \STATE $initPrototype(\mathbcal{S})$
   \STATE $\mathbcal{L}^{'} = merge(\mathbcal{L},\ell)$
   \ENDIF
   \ENDFOR
  
   \UNTIL{$\mathcal{D}$ is empty}
\end{algorithmic}
\end{algorithm}
